Black Box Variational Inference with a Deterministic Objective: Faster, More Accurate, and Even More Black Box

Automatic differentiation variational inference (ADVI) offers fast and easy-to-use posterior approximation in multiple modern probabilistic programming languages. However, its stochastic optimizer lacks clear convergence criteria and requires tuning parameters. Moreover, ADVI inherits the poor posterior uncertainty estimates of mean-field variational Bayes (MFVB). We introduce "deterministic ADVI" (DADVI) to address these issues. DADVI replaces the intractable MFVB objective with a fixed Monte Carlo approximation, a technique known in the stochastic optimization literature as the "sample average approximation" (SAA). By optimizing an approximate but deterministic objective, DADVI can use off-the-shelf second-order optimization, and, unlike standard mean-field ADVI, is amenable to more accurate posterior covariances via linear response (LR). In contrast to existing worst-case theory, we show that, on certain classes of common statistical problems, DADVI and the SAA can perform well with relatively few samples even in very high dimensions, though we also show that such favorable results cannot extend to variational approximations that are too expressive relative to mean-field ADVI. We show on a variety of real-world problems that DADVI reliably finds good solutions with default settings (unlike ADVI) and, together with LR covariances, is typically faster and more accurate than standard ADVI.

==> _math_macros.tex <==
\algblock{Inputs}{EndInputs}
\algnotext{EndInputs}

\algblock{Postprocessing}{EndPostprocessing}
\algnotext{EndPostprocessing}

\newtheorem{assu}{Assumption}
\makeatletter
\if@cref@capitalise
\crefname{assu}{Assumption}{Assumptions}
\else
\crefname{assu}{assumption}{assumptions}
\fi
\Crefname{assu}{Assumption}{Assumptions}
\makeatother

\newtheorem{lem}[theorem]{Lemma}
\makeatletter
\if@cref@capitalise
\crefname{lem}{Lemma}{Lemmas}
\else
\crefname{lem}{lemma}{lemmas}
\fi
\Crefname{lem}{Lemma}{Lemmas}
\makeatother

\newtheorem{ex}{Example}
\makeatletter
\if@cref@capitalise
\crefname{ex}{Example}{Examples}
\else
\crefname{ex}{example}{examples}
\fi
\Crefname{ex}{Example}{Examples}
\makeatother

\newtheorem{defn}{Definition}
\makeatletter
\if@cref@capitalise
\crefname{defn}{Definition}{Definitions}
\else
\crefname{defn}{definition}{definitions}
\fi
\Crefname{defn}{Definition}{Definitions}
\makeatother



% \newtheorem{remark}{Remark}[theorem]
\crefname{remark}{Remark}{Remarks}
\Crefname{remark}{Remark}{Remarks}
% \makeatletter
% \if@cref@capitalise
% \crefname{rem}{Remark}{Remarks}
% \else
% \crefname{rem}{remark}{remarks}
% \fi
% \Crefname{rem}{Remark}{Remarks}
% \makeatother


\newcommand{\dataset}{{\cal D}}
\newcommand{\fracpartial}[2]{\frac{\partial #1}{\partial  #2}}
\newcommand{\fracat}[3]{\left. \frac{#1}{#2} \right|_{#3}}
\newcommand{\trans}{\intercal}
\newcommand{\const}{C}
\newcommand{\diag}[1]{\mathrm{Diag}\left(#1\right)}
\newcommand{\grad}[2]{\nabla_{#1} \left. #2 \right.}
\newcommand{\hess}[2]{\nabla^2_{#1} \left. #2 \right.}
\newcommand{\gradat}[3]{\nabla_{#1} \left. #2 \right|_{#3}}
\newcommand{\norm}[1]{\left\Vert #1\right\Vert}
\newcommand{\abs}[1]{\left| #1\right|}
\newcommand{\normp}[1]{\left\Vert #1\right\Vert_*}
\newcommand{\trace}[1]{\mathrm{Tr}\left(#1\right)}
\newcommand{\oned}[1][\thetadim]{1_{#1}} % Vector of ones
\newcommand{\zerod}[1][2\thetadim]{0_{#1}} % Vector of zeros
\newcommand{\ident}[1][\thetadim]{I_{#1}} % Identity matrix
\newcommand{\dequal}{\stackrel{d}{=}}


\newcommand{\y}{y}  % data
\newcommand{\z}{Z}  % Reparameterization trick variable
\newcommand{\Z}{\mathscr{Z}}  % Set of \z
\newcommand{\znum}{N} % Number of elements of \Z
\newcommand{\Zindep}{\tilde{\Z}}  % Set of \z
\newcommand{\p}{\mathcal{P}} % posterior and model probability
\newcommand{\q}{\mathcal{Q}} % vb approximation
\newcommand{\gfull}{\mathcal{G}} % Grad of exact KL
\newcommand{\g}{\hat{\gfull}} % Grad of MC KL
\newcommand{\hfull}{\mathcal{H}} % Hess of exact KL
\newcommand{\h}{\hat{\hfull}} % Hess of MC KL
\newcommand{\scorecov}{\hat{\Sigma}_{s}} % Estimated score covariance
\newcommand{\fun}{f} % Function of interest
\newcommand{\etahat}{\hat{\eta}}
\newcommand{\etatil}{\tilde{\eta}}
%\newcommand{\etastar}{\stackrel{*}{\eta}} % Superscripts are too high
%\newcommand{\etastar}{\eta^{*}} % Double superscript
\newcommand{\etastar}{\accentset{*}{\eta}}
\newcommand{\ghat}{\hat{g}} % MC estimate of model grad
\newcommand{\hhat}{\hat{h}} % MC estimate of model hessian


\newcommand{\qoi}[1]{\phi\left(#1\right)}
\newcommand{\qoigrad}[1]{\nabla_{\eta} \phi\left(#1\right)}
\def\normal#1#2{\mathcal{N}\left(#1 \vert #2\right)}
\def\wishart#1#2{\mathcal{W}\left(#1 \vert #2\right)}
\def\normz{\mathcal{N}_{\mathrm{std}}\left(\z\right)}
\newcommand{\post}{\p(\theta \vert \y)}
\newcommand{\logjoint}{\log \p(\theta, \y)}
\newcommand{\etaopt}{\hat{\eta}}
% \newcommand{\etaoptd}{\hat{\eta}_{D}}
% \newcommand{\etaopts}{\hat{\eta}_{S}}

% https://stackoverflow.com/questions/1812214/latex-optional-arguments
\newcommand{\etamu}[1][]{\mu_{#1}}
\newcommand{\etamuhat}[1][]{\hat{\mu}_{#1}}
\newcommand{\etamustar}[1][]{\accentset{*}{\mu}_{#1}}

\newcommand{\etasigma}[1][]{\sigma_{#1}}
\newcommand{\etasigmahat}[1][]{\hat{\sigma}_{#1}}
\newcommand{\etasigmastar}[1][]{\accentset{*}{\sigma}_{#1}}

\newcommand{\etaxi}[1][]{\xi_{#1}}
\newcommand{\etaxihat}[1][]{\hat{\xi}_{#1}}
\newcommand{\etar}[1][]{{R_{#1}}}

\newcommand{\qdom}{\Omega_{\q}}
\newcommand{\thetadom}{\Omega_{\theta}}
\newcommand{\rdom}[1]{\mathbb{R}^{#1}}
\newcommand{\etadom}{\Omega_{\eta}}

\newcommand{\thetadim}{D_{\theta}}
\newcommand{\etadim}{D_{\eta}}
\newcommand{\lambdadim}{D_{\lambda}}
\newcommand{\gammadim}{D_{\gamma}}

\def\expect#1#2{\underset{#1}{\mathbb{E}}\left[#2\right]}
\newcommand{\meanz}{\frac{1}{\znum} \sum_{n=1}^{\znum}}
\def\sumn{\sum_{n=1}^{N}}
\def\meann{\frac{1}{N}\sumn}
\def\sump{\sum_{p=1}^{P}}
\def\sumd{\sum_{d=1}^{\thetadim}}
\def\meann{\frac{1}{N}\sumn}
\def\expecthat#1#2{\underset{#1}{\widehat{\mathbb{E}}}\left[#2\right]}
\def\var#1#2{\underset{#1}{\mathrm{Var}}\left(#2\right)}
\def\varhat#1#2{\underset{#1}{\widehat{\mathrm{Var}}}\left(#2\right)}
\def\lrcovfull#1#2{\underset{#1}{\mathrm{LRCov}}\left(#2\right)}
\def\lrcov#1#2{\underset{#1}{\widehat{\mathrm{LRCov}}}\left(#2\right)}
\def\lrvar#1#2{\underset{#1}{\mathrm{LRVar}}\left(#2\right)}
\def\cov#1#2{\underset{#1}{\mathrm{Cov}}\left(#2\right)}

\def\kl#1#2{\mathscr{L}\left(#1 || #2\right)}
\def\klfullobj#1{\mathscr{L}_{\mathrm{VI}}\left(#1\right)}
\def\klobj#1{\widehat{\mathscr{L}}_{\mathrm{VI}}\left(#1\right)}

\def\expectpost#1{\expect{\post}{#1}}

% High dimensional normals notation
\def\zbar{\bar{z}}
\def\zzbar{\overline{zz^\trans}}
\def\sigmat{S}
\def\zcov{\hat{\Sigma}_{z}}


\DeclareMathOperator*{\argmax}{\mathrm{argmax}}
\DeclareMathOperator*{\argmin}{\mathrm{argmin}}
\DeclareMathOperator*{\esssup}{\mathrm{esssup}}
\DeclareMathOperator*{\essinf}{\mathrm{essinf}}
\DeclareMathOperator*{\argsup}{\mathrm{argsup}}
\DeclareMathOperator*{\arginf}{\mathrm{arginf}}

% Experiment results

\def\method{\textrm{\tiny METHOD}}
\def\nuts{\textrm{\tiny NUTS}}
\def\sadvi{\textrm{\tiny MF-ADVI}}
\def\sadvifr{\textrm{\tiny FR-ADVI}}
\def\raabbvi{\textrm{\tiny RAABBVI}}
\def\dadvi{\textrm{\tiny DADVI}}
\def\lrvb{\textrm{\tiny LRVB}}

\def\muerr{\varepsilon^{\mu}}
\def\sderr{\varepsilon^{\sigma}}
\def\freqsd{\xi}
\def\freqerr{\varepsilon^{\xi}}

\def\zbar{\bar{z}}
\def\zzbar{\overline{zz^\trans}}
\def\sigmat{S}
\def\zcov{\hat{\Sigma}_{z}}


==> methods_intro.tex <==
In what follows, we start by establishing the requisite notation and 
the various forms of automatic differentiation variational inference (ADVI).
Then we introduce our new method 
``deterministic automatic differentiation variational inference'' (DADVI),
describe how it facilitates LR
covariances, and show how to compute its Monte Carlo error.
